Generalizable Visual Reinforcement Learning with Segment Anything Model

Learning policies that can generalize to unseen environments is a fundamental challenge in visual reinforcement learning (RL). While most current methods focus on acquiring robust visual representations through auxiliary supervision, pre-training, or data augmentation, the potential of modern vision foundation models remains underleveraged. In this work, we introduce Segment Anything Model for Generalizable visual RL (SAM-G), a novel framework that leverages the promptable segmentation ability of Segment Anything Model (SAM) to enhance the generalization capabilities of visual RL agents. We utilize image features from DINOv2 and SAM to find correspondence as point prompts to SAM, and then SAM produces high-quality masked images for agents directly. Evaluated across 8 DMControl tasks and 3 Adroit tasks, SAM-G significantly improves the visual generalization ability without altering the RL agents' architecture but merely their observations. Notably, SAM-G achieves 44% and 29% relative improvements on the challenging video hard setting on DMControl and Adroit respectively, compared to state-of-the-art methods. Video and code: https://yanjieze.com/SAM-G/

==> tables/ablation_no_3_weight.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation on PerSAM adaptation.} \ours adopts the efficient parameter finetuning technique from PerSAM~\citep{zhang2023persam} which only takes ~10 seconds. We ablate on the necessity of this design and observe that this adaptation is generally helpful.}
\label{table:ablation 3 weights}
\vspace{-0.1in}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccc|cc}
\toprule


Ablations & Walker  & Cartpole  & Finger & Ball\_in\_cup  & \multirow{2}{*}{\textbf{Average}}\\
(color hard) &walk & swingup & spin & catch \\
 
\midrule
\ours & \dd{805}{37}& \dd{728}{51}& \dd{739}{32}& \dd{949}{26} & $805$ \\
w/o. PerSam adapt & \dd{659}{93} & \dd{501}{28} & \dd{833}{136} & \dd{894}{91} & $722$ \down{172} \\


\bottomrule
\end{tabular}}

\vspace{0.05in}

\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccc|cc}
\toprule


DMControl & Walker  & Cartpole  & Finger & Ball\_in\_cup  & \multirow{2}{*}{\textbf{Average}}\\
(video easy) &Walk & Swingup & Spin & Catch \\
 
\midrule
\textbf{\ours} & \dd{887}{33}& \dd{855}{6}& \dd{937}{21}& \dd{858}{79} & $884$ \\
w/o. PerSam adapt & \dd{817}{35} & \dd{469}{75} & \dd{939}{42} & \dd{911}{56} & $784$ \down{100} \\


\bottomrule
\end{tabular}}

\vspace{0.05in}

\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccc|cc}
\toprule

DMControl & Walker  & Cartpole  & Finger & Ball\_in\_cup  & \multirow{2}{*}{\textbf{Average}}\\
(video hard) &Walk & Swingup & Spin & Catch \\
 
\midrule
\textbf{\ours} & \dd{870}{28}& \dd{747}{5}& \dd{932}{22}& \dd{771}{101} & $830$\\
w/o. PerSam adapt & \dd{803}{26} & \dd{336}{107} & \dd{919}{22} & \dd{802}{112} & $715$ \down{115}\\

\bottomrule
\end{tabular}}

\end{table}

==> tables/ablations_color_hard.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Color hard on DMControl.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccc|cc}
\toprule


Ablations & Walker  & Cartpole  & Finger & Ball\_in\_cup  & \multirow{2}{*}{\textbf{Average}}\\
(color hard) &walk & swingup & spin & catch \\
 
\midrule
\ours & \dd{805}{37}& \dd{728}{51}& \dd{739}{32}& \dd{949}{26} & $805$ 
\\w/o. DINOv2 &   \dd{726}{39}&  \dd{589}{75} & \dd{785}{90}& \dd{921}{10} & $753$
\\w/o. extra points &  \dd{761}{64} & \dd{649}{78} & \dd{783}{34}& \dd{929}{17} & $781$
\\w/o. refinement & \dd{708}{73} \\

\bottomrule
\end{tabular}}
\end{table}



==> tables/ablations_video_easy.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Video easy on DMControl.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccc|cc}
\toprule


Ablations & Walker  & Cartpole  & Finger & Ball\_in\_cup  & \multirow{2}{*}{\textbf{Average}}\\
(video easy) &walk & swingup & spin & catch \\
 
\midrule
\ours & \dd{887}{33}& \dd{855}{6}& \dd{937}{21}& \dd{858}{79} & $884$
\\w/o. DINOv2 &   \dd{871}{13}&  \dd{611}{82} & \dd{949}{15}& \dd{706}{59} & $784$
\\w/o. extra points &  \dd{843}{55} & \dd {659}{58} & \dd{930}{24}& \dd {885}{18} & $829$
\\w/o. refinement & \dd{834}{136}  \\

\bottomrule
\end{tabular}}
\end{table}



==> tables/ablations_video_hard.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Video hard on DMControl.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccc|cc}
\toprule


Ablations & Walker  & Cartpole  & Finger & Ball\_in\_cup  & \multirow{2}{*}{\textbf{Average}}\\
(video hard) &walk & swingup & spin & catch \\
 
\midrule
\ours & \dd{870}{28}& \dd{747}{5}& \dd{932}{22}& \dd{771}{101} & $830$
\\w/o. DINOv2 &   \dd{782}{27}&  \dd{307}{61} & \dd{862}{22}& \dd{404}{97} & $589$
\\w/o. extra points &  \dd{805}{41} & \dd {491}{45}  & \dd{688}{11}& \dd{847}{53} & $708$
\\w/o. refinement & \dd{819}{140} & & & & \\

\bottomrule
\end{tabular}}
\end{table}



==> tables/adroit_color_easy.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Color Easy on Adroit.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule



Adroit  &  \multirow{2}{*}{VRL3} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{SGQN} & \multirow{2}{*}{PIE-G} & PIE-G\\
 (color easy)& & & &  & + \ours &\\
\midrule
Pen & \dd{0.1}{0.0} & \dd{55.0}{8.6} & \dd{51.4}{18.1} & \dd{70.6}{2.9} & \dd{60.0}{12.8}\\
Door & \dd{0.0}{0.0} & \dd{45.4}{9.7} & \dd{58.2}{12.9} & \dd{81.6}{6.7} & \dd{96.0}{3.6}\\
Hammer & \dd{0.0}{0.0}  & \dd{24.0}{15.6} & \dd{75.0}{8.6}& \dd{45.8}{19.3} & \dd{88.0}{9.3}\\

\midrule
\textbf{Average} & $0.0$ & $41.5$ & $61.5$ & $66.0$ & $81.3$ \\
\bottomrule
\end{tabular}}
\end{table}

==> tables/adroit_color_hard.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Color Hard on Adroit.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule


Adroit  &  \multirow{2}{*}{VRL3} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{SGQN} & \multirow{2}{*}{PIE-G} & PIE-G\\
 (color hard)& & & &  & + \ours &\\
\midrule
 
Pen & \dd{0.1}{0.0} & \dd{47.0}{6.8} & \dd{36.8}{13.7} & \dd{57.4}{4.2} & \dd{53.0}{5.0}\\
Door & \dd{0.0}{0.0} & \dd{11.8}{3.6} & \dd{31.4}{9.8} & \dd{67.8}{9.8} & \dd{90.3}{4.2}\\
Hammer & \dd{0.0}{0.0} & \dd{9.0}{6.3} & \dd{27.8}{6.4} & \dd{53.2}{12.5} & \dd{60.0}{12.8}\\
\midrule
\textbf{Average} & $0.0$& $22.6$& $32.0$& $59.5$& $67.8$\\

\bottomrule
\end{tabular}}
\end{table}

==> tables/adroit_video_easy.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Video Easy on Adroit.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule


Adroit  &  \multirow{2}{*}{VRL3} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{SGQN} & \multirow{2}{*}{PIE-G} & PIE-G\\
 (video easy)& & & &  & + \ours &\\
\midrule
 
Pen & \dd{0.0}{0.0} & \dd{50.2}{8.6} & \dd{51.4}{18.1} & \dd{67.0}{8.8} & \dd{61.3}{9.3} \\
Door & \dd{0.0}{0.0} & \dd{44.8}{8.5} & \dd{58.2}{12.3} & \dd{81.6}{4.4} & \dd{98.0}{1.0} \\
Hammer & \dd{0.0}{0.0}  & \dd{8.4}{8.6} & \dd{61.0}{9.4} & \dd{50.4}{21.2} & \dd{83.3}{7.0} \\
\midrule
\textbf{Average} & $0.0$& $34.5$& $61.5$& $66.3$& $80.9$\\

\bottomrule
\end{tabular}}
\end{table}

==> tables/adroit_video_hard.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Video Hard on Adroit.}  }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule


Adroit  &  \multirow{2}{*}{VRL3} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{SGQN} & \multirow{2}{*}{PIE-G} & PIE-G\\
 (video hard)& & & &  & + \ours &\\
\midrule
 
Pen & \dd{3.6}{0.9} & \dd{46.8}{9.7} & \dd{54.0}{3.7} & \dd{56.6}{6.3} & \dd{55.3}{4.2} \\
Door & \dd{0.0}{0.0} & \dd{7.6}{1.8} & \dd{21.6}{6.4} & \dd{60.4}{12.3} & \dd{88.3}{3.1} \\
Hammer & \dd{0.0}{0.0} & \dd{4.2}{3.7} & \dd{19.2}{7.4} & \dd{52.6}{10.2} & \dd{58.7}{11.2} \\
\midrule
\textbf{Average}& $1.2$& $19.5$& $31.6$& $56.5$& $67.4$\\

\bottomrule
\end{tabular}}
\end{table}

==> tables/dmc_color_easy.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Color easy on DMControl.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule



DMControl  &  \multirow{2}{*}{DrQ-v2} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{PIE-G} & DrQ-v2 & PIE-G\\
 Color Easy& & & & + \ours  & + \ours &\\
\midrule
Task1 & \\
Task2 &   \ddbf{666}{66}\\
Task3 &  \ddbfblue{888}{88} \\
Task4 & \dd{888}{88} \\

\bottomrule
\end{tabular}}
\end{table}



==> tables/dmc_color_hard.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Color hard on DMControl.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule


DMControl  &  \multirow{2}{*}{DrQ-v2} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{PIE-G} & DrQ-v2 & PIE-G\\
 (color hard)& & & & + \ours  & + \ours &\\
\midrule
Walker walk & \dd{168}{90} & \dd{760}{145} & \dd{884}{20} & \dd{805}{37} & \dd{895}{24}\\
Walker stand & \dd{413}{61} & \dd{942}{26} & \dd{960}{15} &\dd{839}{80}  & \dd{971}{4} \\
Cartpole swingup & \dd{277}{80} & \dd{837}{23} & \dd{749}{46} & \dd{728}{15} & \\
Cheetah run & \dd{109}{45} & \dd{273}{23} & \dd{369}{53} & \dd{280}{48} & \\
Hopper stand & \dd{383}{41} & \dd{715}{78} & \dd{681}{72} &\dd{839}{80} & \\
Finger spin & \dd{676}{134} & \dd{977}{5} & \dd{882}{69} & \dd{740}{32} & \dd{935}{66}\\
Ball\_in\_cup catch & \dd{469}{99} & \dd{961}{7} & \dd{964}{7} & \dd{949}{26} & \\
Quadruped walk & \dd{162}{40} & \dd{879}{8} & \dd{822}{8} & \dd{893}{19} & \dd{759}{44} \\
\midrule
\textbf{Average} & $332$ & $793$ & $789$ &  \\
\bottomrule
\end{tabular}}
\end{table}



==> tables/dmc_video_easy.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Video easy on DMControl.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule



DMControl  &  \multirow{2}{*}{DrQ-v2} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{PIE-G} & DrQ-v2 & PIE-G\\
 (video easy)& & & & + \ours  & + \ours &\\
\midrule
Walker walk & \dd{175}{117} & \dd{819}{71} & \dd{871}{22} & \dd{887}{33} & \dd{930}{28}\\
Walker stand & \dd{560}{48} & \dd{961}{8} & \dd{957}{12} & \dd{971}{2} & \dd{970}{7} \\
Cartpole swingup & \dd{267}{41} & \dd{782}{27} & \dd{587}{61} & \dd{855}{7} & \\
Cheetah run & \dd{64}{22} & \dd{249}{20} & \dd{287}{20} & & \\
Hopper stand & \dd{261}{62} & \dd{678}{30} & \dd{514}{51} &\dd{971}{2} & \\
Finger spin & \dd{456}{15} & \dd{808}{33} & \dd{837}{107} & \dd{937}{21} & \dd{928}{65} \\
Ball\_in\_cup catch & \dd{454}{60} & \dd{871}{106} & \dd{922}{20} & \dd{858}{79} & \\
Quadruped walk & \dd{681}{29} & \dd{818}{6} & \dd{805}{14} & \dd{916}{14} & \dd{789}{72} \\
\midrule
\textbf{Average} & $365$  & $748$ & $723$\\
\bottomrule
\end{tabular}}
\end{table}



==> tables/dmc_video_hard.tex <==

\begin{table}[t]
\centering
\caption{\textbf{Video Hard on DMControl.} }
\label{table:dmc}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule


DMControl  &  \multirow{2}{*}{DrQ-v2} & \multirow{2}{*}{SVEA} & \multirow{2}{*}{PIE-G} & DrQ-v2 & PIE-G\\
 (video hard)& & & & + \ours  & + \ours &\\
\midrule
Walker walk & \dd{34}{11} & \dd{377}{93} & \dd{600}{28} & \dd{846}{38} & \dd{857}{31}\\
Walker stand & \dd{151}{13} & \dd{834}{46} & \dd{852}{56} &\dd{966}{2} & \dd{964}{4} \\
Cartpole swingup & \dd{130}{3} & \dd{393}{45} & \dd{401}{21} & \dd{747}{5} & \\
Cheetah run & \dd{23}{5} & \dd{105}{37} & \dd{154}{17} & & \\
Hopper stand & \dd{5}{5} &\dd{221}{13} & \dd{235}{17}&\dd{840}{30} & \\
Finger spin & \dd{21}{4} & \dd{335}{58} & \dd{762}{59} & \dd{932}{22} & \dd{908}{66} \\
Ball\_in\_cup catch & \dd{97}{27} & \dd{403}{174} & \dd{786}{47} & \dd{771}{101} & \\
Quadruped walk & \dd{69}{21} & \dd{532}{23} & \dd{483}{62} & \dd{774}{22} & \dd{635}{21} \\
\midrule
\textbf{Average}\\
\bottomrule
\end{tabular}}
\end{table}



==> tables/pen_highresolution.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Using higher resolution for pen.} We increase the resolution of the visual observation from $84\times 84$ to $160\times 160$.}
\label{table:pen high resolution}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lccccc|c}
\toprule


Pen &  \multirow{2}{*}{Train} & Color & Color  & Video & Video & \multirow{2}{*}{\textbf{Average}}\\

high resolution & & easy & hard & easy & hard \\
 
\midrule
VRL3 & \dd{88.0}{9.9} & \dd{1.7}{0.7} & \dd{3.7}{2.1} & \dd{1.7}{0.6} & \dd{2.7}{1.5} & $19.6$\\
SVEA & \dd{67.7}{11.7} & \dd{53.3}{7.6} & \dd{44.7}{5.8} & \dd{46.7}{3.8} & \dd{41.7}{6.1} & $50.8$\\
SGQN & \dd{86.7}{1.5} & \dd{71.3}{5.0} & \dd{54.3}{7.1} & \dd{68.7}{8.1} & \dd{52.3}{0.6} & $66.7$\\
PIE-G & \dd{79.7}{6.1} & \dd{76.0}{7.0} & \dd{70.3}{4.6} & \dd{76.0}{1.7} & \dd{60.7}{6.0} & $72.5$\\
\textbf{\ours} & \dd{82.0}{10.5} & \dd{79.0}{4.4} & \dd{75.3}{6.7} & \dd{82.3}{5.1} & \dd{76.7}{2.1} & $79.6$\\


\bottomrule
\end{tabular}}
\end{table}
